RLIBM-32: High Performance Correctly Rounded Math Libraries for 32-bit Floating Point Representations

This paper proposes a set of techniques to develop correctly rounded math libraries for 32-bit float and posit types. It enhances our RLibm approach that frames the problem of generating correctly rounded libraries as a linear programming problem in the context of 16-bit types to scale to 32-bit types. Specifically, this paper proposes new algorithms to (1) generate polynomials that produce correctly rounded outputs for all inputs using counterexample guided polynomial generation, (2) generate efficient piecewise polynomials with bit-pattern based domain splitting, and (3) deduce the amount of freedom available to produce correct results when range reduction involves multiple elementary functions. The resultant math library for the 32-bit float type is faster than state-of-the-art math libraries while producing the correct output for all inputs. We have also developed a set of correctly rounded elementary functions for 32-bit posits.

==> fig.workflow.tex <==
\begin{figure*}[t]
%\vspace*{-4mm}
\begin{overpic}[width=\textwidth]{figures/overview.pdf}
    \put(3,8){Input in $\mathbb T$}
    \put(14.5,8){\tiny Sample}
    \put(21,8){Sampled input}
    \put(25,6){in $\mathbb T$}
    \put(35,8){\tiny Convert}
    \put(41.5,8){Sampled input}
    \put(45.5,6){in $\mathbb H$}
    \put(56,8.5){\tiny Range}
    \put(55,7.5){\tiny Reduction}
    \put(63.5,8){Reduced}
    \put(63,6){input in $\mathbb H$}
    \put(82,.5){\small Generate Piecewise}
    \put(85,-1.2){\small Polynomials}
    \put(82,-2.9){\small using our method}
    \put(65.5,-1){Reduced}
    \put(63.5,-3){intervals in $\mathbb H$}
    \put(55.5,-.5){\tiny Reverse}
    \put(55.5,-1.5){\tiny Output}
    \put(53.5,-2.5){\tiny Compensation}
    \put(42.5,-1){Rounding}
    \put(41,-3){intervals in $\mathbb H$}
    \put(21,-1){Identify values}
    \put(23,-3){in $\mathbb H$ that}
    \put(22.5,-5){round to $y$}
    \put(2,-1){$y=$ Correctly}
    \put(0,-3){rounded $f(x)\in\mathbb T$}
\end{overpic}
\vspace*{.1mm}
\caption{Overview.}
\vspace*{-5mm}
\label{fig:workflow}
\end{figure*}

